PrismaCoder: Pushing the Boundaries of Open Multimodal Code Intelligence through Decomposed Rubric Synthesis

Multimodal code intelligence connects the symbolic world of programs with the visual world their execution creates. Interest in this capability is burgeoning, as models are increasingly asked to produce charts, webpages, animations, and semi-structured documents. Recently, proprietary models have pushed far ahead, producing interactive artifacts even from a text description or a screenshot alone. Yet their data and training remain closed, and open progress is held back by the quantity and quality of available data and by the pipelines and methods for producing it. Quality is the harder of the two, since a sample must be correct as a program, well built, and above all visually right once rendered. No existing signal covers all three. Execution often returns just a pass or fail, code similarity does not map to the visual output, and task-specific verifiers do not generalize. To push open progress further, we start from the data side with PrismaForge, a hierarchical data pipeline centered on a synthesized rubric that decomposes these factors into checkable criteria. The same rubric serves as both filter and reward: it curates the supervised corpus, then drives reinforcement learning on visual-coding tasks. Leveraging PrismaForge for data synthesis and filtering, we build PrismaCoder-2M, the most diverse open dataset for multimodal code intelligence and the largest to date. On the model side, we train PrismaCoder-9B and PrismaCoder-35B on this data and release both. They lead the open state of the art by a wide margin and rival leading proprietary systems. Our analyses further show that the proposed rubric-based pipeline improves multimodal coding performance across model backbones. We release our code and data at https://qiushisun.github.io/PrismaCoder-Home/.

==> zytxnxngzdvxqhckpnjsbqvcvffzphrh/Appendices/acknowledgments.tex <==
\section*{Acknowledgments}
\label{sec:ack}

This research is supported by the WYNG Foundation (HKU 25AG100407).
We thank Xiao Wang for advice on molecular generation and Xuanle Zhao for
guidance on reproducing the baselines.


==> zytxnxngzdvxqhckpnjsbqvcvffzphrh/Figures/data_pie.tex <==
\begin{figure}[t]
\begin{minipage}[c]{0.47\linewidth}
\centering
\captionof{table}{Statistics of \ourdata{}.}
\label{tab:data-stats}
\footnotesize
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{0.9}
\begin{tabular}{l r r}
\toprule
Task family & \#Samples & Share \\
\midrule
\multicolumn{3}{l}{\swatch{pievision}\textit{Vision-centric}} \\
WebUI Generation      & 357.1K & 17.8\% \\
Chart-to-Code         & 196.5K &  9.8\% \\
Image-to-SVG          & 181.0K &  9.0\% \\
WebUI Editing         & 175.0K &  8.7\% \\
Demo / Artifacts      & 163.3K &  8.1\% \\
Chemical Structures   & 108.0K &  5.4\% \\
Interactive Artifacts &   9.1K &  0.5\% \\
\midrule
\multicolumn{3}{l}{\swatch{pietext}\textit{Text-centric}} \\
Chart Generation      & 181.1K &  9.0\% \\
Demo / Artifacts      & 163.0K &  8.1\% \\
Text-to-WebUI         & 135.2K &  6.7\% \\
\LaTeX{}              & 133.1K &  6.6\% \\
SVG Generation        &  53.3K &  2.7\% \\
Animation (Manim)     &  35.9K &  1.8\% \\
JavaScript            &  28.5K &  1.4\% \\
Mermaid               &  22.7K &  1.1\% \\
LilyPond              &  21.9K &  1.1\% \\
Vega-Lite             &  20.0K &  1.0\% \\
Asymptote             &  19.4K &  1.0\% \\
\midrule
Total                 & 2M & 100\% \\
\bottomrule
\end{tabular}
\end{minipage}\hfill
\begin{minipage}[c]{0.50\linewidth}
\centering
\includegraphics[width=\linewidth]{Figures/data_pie/prismacoder_data_pie.pdf}
\caption{Composition of \ourdata{} by input modality and task family.}
\label{fig:data-pie}
\end{minipage}
\vspace{-1em}
\end{figure}


==> zytxnxngzdvxqhckpnjsbqvcvffzphrh/Figures/pipeline.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.95\linewidth]{Figures/pipeline.pdf}
\caption{\pipename{} writes one rubric per instruction and uses it twice, to filter
candidate data into \ourdata{} and to reward rollouts in reinforcement learning.}
\label{fig:pipeline}
\end{figure}


==> zytxnxngzdvxqhckpnjsbqvcvffzphrh/Figures/rubric_example.tex <==
\begin{figure}[t]
\centering
\setlength{\fboxsep}{0pt}\setlength{\fboxrule}{0.4pt}
\begin{minipage}[c]{0.36\linewidth}\centering
\fcolorbox{black!30}{white}{\includegraphics[height=1.36in]{Figures/appendix/rubric_case_1_gold.png}}\\[3pt]
{\footnotesize Reference}
\end{minipage}\hfill
\begin{minipage}[c]{0.31\linewidth}\centering
\fcolorbox{black!30}{white}{\includegraphics[height=1.36in]{Figures/appendix/rubric_case_1_synthesis.png}}\\[3pt]
{\footnotesize Synthesized}
\end{minipage}\hfill
\begin{minipage}[c]{0.29\linewidth}\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.3}
\begin{tabular}{@{}lcr@{}}
\toprule
Signal & Checks & Score \\
\midrule
Holistic judge & -- & 78\,/\,100 \\
\rowcolor{figCodeFill} Code rubric & 5\,/\,5 pass & 1.00 \\
\rowcolor{figVisFill} Vision rubric & 1\,/\,5 pass & 0.18 \\
\bottomrule
\end{tabular}
\end{minipage}
\caption{Scored separately, the vision rubric catches a misplaced footer that every code
check and a holistic judge let through.}
\label{fig:rubric-example}
\end{figure}


==> zytxnxngzdvxqhckpnjsbqvcvffzphrh/Figures/task_overview.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.95\linewidth]{Figures/task_overview.pdf}
\caption{Scenarios and formats covered by \ourdata{} and \methodname{}.}
\label{fig:task-overview}
\vspace{-7pt}  
\end{figure}


==> zytxnxngzdvxqhckpnjsbqvcvffzphrh/Sections/0-abstract.tex <==
\begin{abstract}
Multimodal code intelligence connects the symbolic world of programs with the
visual world their execution creates. Interest in this capability is
burgeoning, as models are increasingly asked to produce charts, webpages,
animations, and semi-structured documents. Recently, proprietary models have
pushed far ahead, producing interactive artifacts even from a text description
or a screenshot alone. Yet their data and training remain closed, and
open progress is held back by the quantity and quality of available
data and by the pipelines and methods for producing it. Quality is the harder
of the two, since a sample must be correct as a program, well built, and above
all visually right once rendered. No existing signal covers all three.
Execution often returns just a pass or fail, code similarity does not map to the
visual output, and task-specific verifiers do not generalize. To push open
progress further, we start from the data side with \pipename{}, a hierarchical
data pipeline centered on a synthesized rubric that decomposes these factors
into checkable criteria. The same rubric serves as both
filter and reward: it curates the supervised corpus, then drives
reinforcement learning on visual-coding tasks. Leveraging \pipename{} for data
synthesis and filtering, we build \ourdata{}, the most diverse open dataset for
multimodal code intelligence and the largest to date. On the model side, we train \modelnine{} and
\modelthirtyfive{} on this data and release both. They lead the open state of
the art by a wide margin and rival leading proprietary systems. 
% Our analyses further
% show that our rubric-guided data curation improves downstream performance and that the
% pipeline generalizes across model backbones. 
Our analyses further show that the proposed rubric-based pipeline improves multimodal coding performance across model backbones.
We release our code, model, and data at the
\href{https://qiushisun.github.io/PrismaCoder-Home/}{PrismaCoder Homepage}.
\end{abstract}


==> zytxnxngzdvxqhckpnjsbqvcvffzphrh/Sections/1-intro.tex <==
\section{Introduction}
\label{sec:intro}

\input{Figures/task_overview}

From symbols to pixels, code intelligence now extends beyond textual source code
into the visual world that programs produce~\citep{zan2023large,sun2024survey, zhao2026beyond}. A growing range of applications
specifies intent through images and judges a result by what its code renders, from charts and web pages to
diagrams, typeset documents, and animations. Leading
proprietary systems now produce interactive artifacts from a text description or
a screenshot alone.

Prior open efforts have mostly addressed one corner of this space at a time, from
plotting~\citep{ni2025viscoder, pandasplotbench2025timur, yang2024matplotagent}
and chart-to-code~\citep{yang2025chartmimic, zhao2025chartcoder} to
screenshot-to-page generation~\citep{gui2025webcode2m, si2025design2code}. Each
comes with its own data and recipe,
making it difficult for the resulting models to generalize across task domains and output formats.
Recently, open work such as
JanusCoder~\citep{sun2026januscoder} has brought many of these scenarios under a
shared visual-programmatic interface, with follow-up refinements building on the
same view~\citep{zhao2025vincicoderunifyingmultimodalcode, jiang2026viscodex, ni2026viscoder}.
Despite these advances, publicly available training data remains limited in scale and uneven in quality, with only a handful of open releases and resources to date~\citep{sun2026januscoder, jiang2026viscodex}.
The pipelines used to build these datasets are rarely released, while proprietary systems keep their data and training closed. 
Moreover, existing public data are typically curated with either a single per-sample score, which provides limited diagnostic information about errors, or a task-specific verifier, which does not generalize across tasks.

To address this gap, we introduce \pipename{}, a rubric-based framework for multimodal code data curation and policy optimization. Rather than relying solely on a holistic judgment or a fixed checklist, \pipename{} applies a common evaluation procedure across data sources and task domains while tailoring its criteria to each instruction. Each rubric combines reusable domain-level checks with instruction-specific requirements, with the number of criteria adjusted to the estimated task difficulty. Code-level and visual-level criteria are evaluated separately on the generated program and its rendered artifact, respectively. 
These scores guide data curation and serve as reinforcement learning rewards.

Using \pipename{}, we curate \ourdata{},  the broadest open dataset to date for advancing multimodal code intelligence, spanning more than 12 categories and
10 programming languages with both text-centric and vision-centric data. To build this coverage, we draw seeds from complementary sources: public visual-coding corpora cover common plotting and graphics tasks; research figures and open-source repositories contribute long-tail scientific examples; and web, interactive-demo, and chemical-structure sources broaden the range of artifacts. We then convert the seeds into self-contained tasks, check candidate programs through format-specific execution and rendering, and use instruction-specific rubric scores to filter or refine the resulting examples. This gives the dataset both breadth of coverage and a consistent quality-control process.

To assess whether the breadth of \ourdata{} translates into broad model capability, we develop \modelnine{} and \modelthirtyfive{}.  
Evaluated on a wide range of representative benchmarks, \methodname{} leads the existing open state of the art by a wide margin and matches the proprietary systems to a considerable degree (\cref{sec:experiments}).
Through extensive analyses (\cref{sec:analysis}), we show that the data and pipeline generalize across base models beyond our release. We further show that rubric-guided curation outperforms direct-judge selection and that rubric scores align closely with human judgments.

Our main contributions are summarized as follows:
\begin{itemize}[leftmargin=2em, itemsep=2pt, topsep=0pt, parsep=0pt]
    \item \textbf{Decomposed Rubric Synthesis for Visual-coding Data.} We introduce
    \pipename{}, a principled pipeline whose hierarchically synthesized rubrics
    serve as both filter and reward. Based on it, we curate \ourdata{}, the broadest and largest open
    dataset to date.
    \item \textbf{Open Models that Rival Proprietary Systems.} We build \modelnine{}/35B on
    \ourdata{}, which lead the open state of the art by a wide margin and match or surpass
    leading proprietary systems on charts, front-end pages, and semi-structured documents.
    \item \textbf{Empirical Insights across Data, Modeling, and Training.}
    Beyond data and model contributions, we further share insights through extensive analysis. It shows that our pipeline generalizes across scenarios and backbones and yields artifacts better aligned with human preference.
\end{itemize}


==> zytxnxngzdvxqhckpnjsbqvcvffzphrh/Sections/2-related.tex <==
\section{Related Work}
\label{sec:related}

\paragraph{Multimodal Code Intelligence.}
Code intelligence now extends beyond text-only programming to visual-programmatic tasks, where intent may be visual~\citep{li2024mmcode, zhang2024humanevalv, wang2025codevision} and outputs can be judged only after execution or rendering~\citep{zhao2026beyond}.
On the output side, syntactic validity is insufficient; correctness also depends on layout, semantics, interaction, and editability.
On the input side, reading values and layout off renders remains a perception bottleneck~\citep{masry2022chartqa, wang2024charxiv, xia2025chartx} across vision-language models~\citep{zhang2024tinychart, liu2025perceptionbottleneckvlmschart}.
The tasks run from screenshot-to-code~\citep{gui2025webcode2m, si2025design2code, yun2024webcode} to front-end engineering~\citep{ScreenCoder, zhu2025frontendbench, sun2025fullfront} and generative UI~\citep{zheng2026code2world}; chart generation~\citep{yang2025chartmimic, zhao2025chartcoder, wu2025plot2code} and editing~\citep{zhang2024academicvis, zhao2025chartedit}; SVG and symbolic graphics~\citep{yang2025omnisvg, nishina2024svgeditbench, xu2024symbol} with their structural probes~\citep{qiu2025can, chen2025symbolicgraphics}; and interactive artifacts and code-driven demonstrations~\citep{zhang2025artifactsbench, ku2025theoremexplainagent, sun2025osgenesis}.
Recent generalists unify these domains via JanusCoder's visual-programmatic interface~\citep{sun2026januscoder}, VisCodex's vision--code integration~\citep{jiang2026viscodex}, VisCoder2's agentic visualization coding~\citep{ni2026viscoder}, and VinciCoder's visual reinforcement learning~\citep{zhao2025vincicoderunifyingmultimodalcode}.
Yet a shared modeling interface does not by itself make heterogeneous notions of correctness consistently measurable or usable for training~\citep{zhao2026beyond}.
Complementing this progress, we contribute on the data side, with \ourdata{} spanning the broadest scenarios and open data types.

\paragraph{Learning Signals for Code Generation.}
Conventional code tasks~\citep{zhang2023repocoder} draw training data from instruction synthesis and evolution~\citep{wei2024magicoder,luo2024wizard,luo2025tree}.
For many such tasks, executable tests provide a cheap, reproducible signal for data filtering~\citep{xu2025kodcode, sun2026codeevo} and reinforcement learning~\citep{shao2024deepseekmath, xu2025interactive, zhuo2025bigcodearena}.
Visual outputs break this assumption: successful execution confirms only that the code runs, not that its render is faithful, well composed, or semantically correct~\citep{zhao2026beyond, liu2026visual, guo2025mammothvl}.
Visual benchmarks instead use task-specific render checks for charts~\citep{yang2025chartmimic}, visual and structural similarity for web pages~\citep{si2025design2code}, or judge protocols for interactive artifacts~\citep{zhang2025artifactsbench}; effective individually, these measures do not compose across artifacts.
Recent work moves toward finer supervision, from JanusCoder's single-pass rubric over fixed dimensions~\citep{sun2026januscoder} to VinciCoder's coarse-to-fine rewards~\citep{zhao2025vincicoderunifyingmultimodalcode}. Neither signal is yet both fine enough to localize failures and general enough to cover every task, at curation and at training alike. In this work, one synthesized rubric per instruction serves both roles, filtering the training data and rewarding reinforcement learning across every format we cover.


==> zytxnxngzdvxqhckpnjsbqvcvffzphrh/Sections/3-method.tex <==
\section{PrismaForge}
\label{sec:method}
In this section, we present \pipename{}, a rubric-based scoring framework that lies in the center of our data curation and training pipeline.

\input{Figures/pipeline}

\subsection{Elastic Rubric Scorer}
\label{subsec:rubric}

For a large-scale coding dataset prepared for visualization or demonstration, the key challenge is to determine which candidates are sufficiently correct and useful to retain. Unlike problems with easily verifiable outputs, visualization quality is often specified only implicitly~\citep{wu2025plot2code, yang2025chartmimic}. A single holistic score is therefore hard to verify and offers little insight into why a candidate succeeds or fails~\citep{ye2024iclrw-flask, sun2026januscoder}.

A natural alternative is to evaluate candidates using explicit criteria, but a fixed rubric is too coarse for diverse visualization tasks. Different instructions may prioritize numerical accuracy and axis scales, visual similarity, layout, or artifact editability. A universal rubric must stay broad and may miss the properties most important for a specific example. At the other extreme, manually designing separate rubrics for every visualization instruction would require substantial human effort and is hard to scale.

To balance these two extremes, we introduce a sample-specific rubric system that combines reusable domain-level criteria with criteria synthesized specifically for each instruction.

Formally, let $i \in \{1,\ldots,N\}$ index dataset instances, and let $d_i \in \mathcal{D}$ denote the visualization domain associated with instance $i$. We represent candidate sample $i$ as a tuple $(x_i, c_i, v_i)$ where $x_i$ denotes the instruction, which may contain text and optional visual references; $c_i$ denotes the response code produced for that instruction; and $v_i = \operatorname{Exec}(c_i)$ denotes the visual artifact obtained by executing $c_i$. 

We evaluate each candidate using two complementary sets of rubric criteria: code rubrics $\mathcal{R}_i^{(c)}$, which assess properties that can be verified from $c_i$, and visual rubrics $\mathcal{R}_i^{(v)}$, which assess properties directly observable from $v_i$.

\input{Figures/rubric_example}

\Cref{fig:rubric-example} shows why the two views are kept apart. The synthesized page
carries the reference's content, colors, and layout in its code, so every code check passes.
Its footer, however, is drawn over the Services section and clips the third button. A holistic
judge still rates the page 78 out of 100, above about four fifths of the pool, whereas the
vision rubric scores it 0.18. The checks and judgments behind both scores are listed in
Appendix~\cref{app:prompts}.

Within each modality, we further distinguish between domain-shared and sample-specific criteria. Domain-shared rubrics encode requirements that recur across samples within the same visualization domain, whereas sample-specific rubrics are derived from the instruction $x_i$ and capture requirements unique to the current sample. Thus, for modality $m \in \{c,v\}$,
\begin{equation}
\label{eq:rubric-decomposition}
\mathcal{R}_i^{(m)}
=
\mathcal{R}_{\mathrm{shared}}^{(m)}(d_i)
\cup
\mathcal{R}_{\mathrm{spec}}^{(m)}(x_i).
\end{equation}

Because individual criteria may differ in importance, each rubric item $r \in \mathcal{R}_i^{(m)}$ is assigned a nonnegative, sample-dependent weight $w_{i,r}^{(m)}$.

To score a candidate,
let $f^{(m)}(r,y) \in [0,1]$ denote the judge score indicating how well artifact $y$ satisfies rubric criterion $r$ under modality $m$. The normalized score for modality $m$ is then
\begin{equation}
\label{eq:modality-score}
S_i^{(m)}
=
\frac{1}{
\sum_{r \in \mathcal{R}_i^{(m)}}
w_{i,r}^{(m)}
} \sum_{r \in \mathcal{R}_i^{(m)}}
w_{i,r}^{(m)}
f^{(m)}(r,y_i^{(m)})
\end{equation}

The two modality scores are then combined into an overall sample score with appropriate weighting
\begin{equation}
\label{eq:overall-score}
S_i
=
\lambda_c S_i^{(c)}
+
\lambda_v S_i^{(v)},
\end{equation}
where $\lambda_c,\lambda_v \geq 0$ and $\lambda_c+\lambda_v=1$.

In practice, candidate samples vary substantially in difficulty and complexity, and therefore should not be evaluated with the same number of rubric items. We first assign each instruction $x_i$ a difficulty level $q_i \in \mathcal{Q}$ and use this level to guide rubric generation. Each difficulty band is associated with a bounded range for the number of generated criteria. This allows more complex samples to receive finer-grained evaluation while keeping the rubric compact enough to control judging cost.

\subsection{Rubric-Based Policy Optimization}
\label{subsec:rl}

The same rubric framework can also be used to construct rewards for reinforcement learning. Because rubric scores are normalized within each modality and aggregated using a common scoring rule, they provide a consistent reward scale across samples with different numbers and types of criteria. We therefore use the rubric-based evaluator as a structured reward function during policy optimization.

For each prompt $x_i$, we sample $K$ rollout responses from the behavior policy
\begin{equation}
{c_i^{(1)},\cdots,c_i^{(K)}}
\sim
\pi_{\theta_{\mathrm{old}}}(\cdot \mid x_i).
\end{equation}
Each rollout $c_i^{(k)}$ is executed to obtain the visual artifacts $v_i^{(k)}=\textrm{Exec}\left(c_i^{(k)}\right)$. Rollouts that failed to execute or render receive reward $0$.

The judge model then scores these rollouts. For each successful rollout trajectory $(x_i, c_i^{(k)}, v_i^{(k)})$, we apply its accompany rubrics set $(\mathcal{R}_i^{(c)}, \mathcal{R}_i^{(v)})$ and obtain the aggregated score $s_i^{(k)}$ via Eq.~\ref{eq:modality-score}--Eq.\ref{eq:overall-score}. These scores are then leveraged to compute the within-group normalized advantage
\begin{equation}
\hat{A}_i^{(k)}
=
\frac{
s_i^{(k)}-\mu_i
}{
\sigma_i+\epsilon
}
\end{equation}
where $\mu_i=\frac{1}{K} \sum_{k=1}^{K} s_i^{(k)}$ and $\sigma_i$ denotes the standard deviation of ${s_i^{(k)}}$.

With this reward formulation, the policy can then be optimized with the standard GRPO
clipped objective~\citep{shao2024deepseekmath}. In practice, we also used GSPO objective~\citep{gspo} with Rollout Routing Replay techniques~\citep{ma2025stabilizing} for the MoE models to stabilize experts training.

\section{PrismaCoder-2M}
\label{sec:prisma-data}
\input{Figures/data_pie}

We build \ourdata{} with \pipename{} by collecting seeds from complementary sources, gating
them by rubric score into a supervised corpus, and holding out a subset for reinforcement
learning, where the same rubrics supply the reward.

\subsection{Data Sourcing}
\label{subsec:data-gather-gate}
Multimodal code generation needs several capabilities at once, so we collect four kinds of
seeds that each cover one of them and train on them together (\cref{tab:data-stats,fig:data-pie}).

\paragraph{Visualization Fundamentals.} Visual coding starts from a core of plotting skills,
such as mapping data to axes and marks and composing legends and layered plots. Public plotting
datasets build this foundation with instruction--code and visualization--code pairs in
Python~\citep{hunter2007matplotlib} and in SVG, Mermaid, Vega-Lite, and other visualization
languages~\citep{ni2025viscoder, ni2026viscoder, jiang2026viscodex}.

\paragraph{Diverse Scientific Artifacts.} Scientific work produces more varied visuals than
standard charts, from multi-panel figures to domain-specific encodings. Plotting code from
open-source GitHub repositories and figures from arXiv papers bring this variety into the data,
and an AST-based pass splits long or monolithic scripts into self-contained units.

\paragraph{Front-End Layout and Interaction.} Front-end development asks a model to arrange
many elements on a page and to make them respond to users. Web pages from
WebCode2M~\citep{gui2025webcode2m} and the MCD dataset~\citep{jiang2026viscodex} supply the
layout, while interactive demos supply the behavior. The demos are adapted from prior
releases~\citep{sun2026januscoder} or rewritten from static pages~\citep{laurenccon2024websight}
and complex generation prompts~\citep{luo2026mmmg, ni2025proimage} into tasks of varying
visual, functional, and reasoning complexity.

\paragraph{Symbolic Notation.} Science, mathematics, and music communicate through symbolic
notation, where a single wrong symbol breaks the result. Chemical-structure code seeded from
PubChem~\citep{kim2025pubchem} must describe a valid molecule, and \LaTeX{}, Asymptote, LilyPond, and Manim programs must compile into well-formed
documents, figures, scores, and scenes. The first three formats draw on the same sources as the
plots, and the Manim seeds come from the 3Blue1Brown video code.
See Appendix~\cref{app:sources}.

\subsection{Iterative Data Gating}
\label{subsec:data-gating}

Every seed enters \pipename{} as a candidate $(x_i, c_i, v_i)$. Where a seed lacks working code, a curation model $\mathcal{L}^{C}$ generates it, $c_i \sim \mathcal{L}^{C}(\cdot \mid x_i)$, through a code-data synthesis pipeline. \pipename{} works with any such pipeline, and we use a typical open-source one~\citep{sun2026januscoder}. Each candidate must then compile or render through a per-format gatekeeper, $v_i = \operatorname{Exec}(c_i)$, and candidates that still fail after regeneration are set aside in a repair pool.

A rubric generator $\mathcal{L}^{R}$ assigns each candidate its difficulty level and its code and visual rubrics (\cref{subsec:rubric}), and a separate judge $\mathcal{L}^{J}$ scores the code against $\mathcal{R}_i^{(c)}$ and the render against $\mathcal{R}_i^{(v)}$. The modality scores and the overall score $S_i$ follow Eqs.~\ref{eq:modality-score} and~\ref{eq:overall-score}. We use distinct models for rubric generation and judging so that biases in rubric construction are not reproduced during scoring.

We then gate candidates by their overall scores. Those with $S_i < \tau_1$ are discarded, those with $\tau_1 \leq S_i < \tau_2$ are sent back for re-synthesis, and those with $S_i \geq \tau_2$ are retained in the curated pool.

The synthesis pipeline serves this gate in two ways. It re-rolls the code of a mid-band candidate with the failed rubric items as feedback, and it synthesizes new samples seeded by retained candidates. Both kinds of output re-enter the pipeline at the execution gate and are scored and routed like any other candidate. For the final supervised corpus, we retain a sample only if its score meets the threshold for its domain, $S_i \geq \tau_{d_i}$.

\subsection{RL Data Curation}
\label{subsec:rl-data}
Reinforcement learning draws on a compact set of instructions held out from the supervised
pool, which SFT never sees. Among them we keep the medium or hard instructions on which the
SFT policy sometimes succeeds and sometimes fails. Such instructions sit near the policy's
capability boundary, and their rollouts differ in quality enough to give group-relative
optimization a contrast to learn from, whereas instructions that every rollout passes or
fails provide none.

Formally, let $\pi_{\mathrm{SFT}}$ denote the SFT-tuned policy. For each candidate instance $i$, we draw $K$ independent responses
$c_i^{(k)} \sim \pi_{\mathrm{SFT}}(\cdot \mid x_i)$ and evaluate each rollout using the rubric-based scoring function defined in \cref{subsec:rubric}.
We then measure the informativeness of instance $i$ by the empirical dispersion of its rubric
scores
\begin{equation}
\label{eq:rl-score-variance}
U_i=
\frac{1}{K}
\sum_{k=1}^{K}
\left(S_i^{(k)}-\bar S_i\right)^2,
\quad
\bar S_i
=\frac{1}{K}\sum_{k=1}^{K}S_i^{(k)}.
\end{equation}
A large $U_i$ means that the policy sometimes succeeds and sometimes fails on the same
instruction.

In practice, we run RL on all Python, HTML, and SVG tasks, and for each domain we hold out
20K \emph{medium} or \emph{hard} candidates before SFT. We then draw $K=5$ rollouts per instance from $\pi_{\mathrm{SFT}}$, score
each rollout against its code and visual rubrics, and retain the 5K instances with the
largest $U_i$. RL thus concentrates on the policy's capability frontier at a fraction
of the rollout cost of a larger candidate pool.


==> zytxnxngzdvxqhckpnjsbqvcvffzphrh/Sections/4-experiments.tex <==
\section{Experiments}
\label{sec:experiments}

\subsection{Experimental Setup}
\label{subsec:settings}

\paragraph{Models.} We release \modelnine{} and \modelthirtyfiveA{} (abbreviated as \modelthirtyfive{}), post-trained from
Qwen3.5-9B and Qwen3.5-35B-A3B~\citep{qwen3_5}. We also train
Gemma-4-31B-it~\citep{google2026gemma} and Qwen3-VL-30B-A3B-Instruct~\citep{bai2025qwen3}.
More training details are in Appendix~\cref{app:training}.

\paragraph{Data Pipeline Details.} 
We reprocess data from prior open releases~\citep{sun2026januscoder, jiang2026viscodex, ni2026viscoder}. \pipename{} treats its
models as pluggable, and in this paper we use \claudeopus{}~\citep{anthropic2026opus46} as the
curation model and \geminipro{}~\citep{gemini2025gemini3} as the rubric generator. Both data gating
and reinforcement learning use Gemini 3 Flash as the judge.
The sources are listed per category in Appendix~\cref{app:sources}.

\paragraph{Baselines.} Besides Qwen3.5, we compare against open multimodal code models, namely JanusCoderV~\citep{sun2026januscoder}, VinciCoder~\citep{zhao2025vincicoderunifyingmultimodalcode}, and VisCoder2-7B~\citep{ni2026viscoder}.

\subsection{Benchmarking}
\label{subsec:benchmarks}

\paragraph{Vision-Centric Settings.} The vision-centric suite comprises
ChartMimic~\citep{yang2025chartmimic}, WebCode2M~\citep{gui2025webcode2m},
DesignBench~\citep{xiao2025designbench}, Design2Code~\citep{si2025design2code}, and
ChemDraw~\citep{zhao2025vincicoderunifyingmultimodalcode}, together with the image-conditioned
lenses of InteractScience~\citep{chen2025interact} (VQT) and UniSVG~\citep{li2025unisvg} (ISVGen).

\paragraph{Text-Centric Settings.} The text-centric suite comprises
ArtifactsBench~\citep{zhang2025artifactsbench}, PandasPlotBench~\citep{pandasplotbench2025timur},
and VisPlotBench~\citep{ni2026viscoder} in eight visualization languages, together with
InteractScience's programmatic lens (PFT) and UniSVG's text-conditioned lens (TSVGen).

\paragraph{Evaluation Protocol.} Evaluation follows each benchmark's official protocol, with
deterministic metrics reported alongside judge scores. Since some designated judges share a
model family with our pipeline, we check that the gains hold across judges
(\cref{subsec:reliability}). Details are presented in \cref{app:benchmarks}.

\subsection{Vision-Centric Results}
\label{subsec:results-vision}

\paragraph{Web Interfaces.} 
\modelnine{} and \modelthirtyfive{} lead open baseline on front-end generation, achieving judge scores more than 20 points higher than those of task-specific open baselines (\cref{tab:main-vision}). 
\modelnine{} also scores above proprietary model on DesignBench generation and WebCode2M CLIP score. DesignBench editing is the only web-interface metric on which both models score below all Claude 4.6 and Gemini 3 variants.
\input{Tables/main_vision} 

\paragraph{Data Visualization.} On ChartMimic, both of our models lead all open baselines. Specifically, \modelthirtyfive outperforms most proprietary models under both settings. Notably, our 9B model demonstrates the most substantial improvement over its base (the lowest among all evaluated models) and even surpasses most proprietary models. 
This clearly demonstrates the quality and utility of our data.
In addition, the low-level score evaluates rendered text, layout, chart type, and color fidelity, which means our model is more capable of generating those details.


\paragraph{Scientific and Vector Graphics.} On chemical-structure code, \modelthirtyfive{} parses
every output and reaches the highest Tanimoto similarity in the table (97.56). On
InteractScience's visual lens both models lead the open baselines, while
image-conditioned SVG is the one vision-centric column led by an open baseline, VinciCoder-8B. Full per-benchmark metrics are presented in
Appendix~\cref{app:results}, and a chart-to-code case across training stages in Appendix~\cref{app:cases}.

\subsection{Text-Centric Results}
\input{Tables/main_text}

\paragraph{Interactive Applications and Plots.} 
On ArtifactsBench, both models exceed all open baselines and \gptfouro{} on the overall score (\cref{tab:main-text}). On InteractScience's programmatic lens, \modelthirtyfive{} scores 28.00, above the best open baseline and comparable to Gemini 3 Flash. Scaling from 9B to 35B raises the InteractScience PFT score by 3.20 points.

\paragraph{Long-Tail Visual Languages.} 
\modelthirtyfive{} leads open baselines on all three VisPlotBench metrics (\cref{tab:main-text}). Its Mean score is 11.02 points above their best, comparable to Claude Sonnet 4.6.

\label{subsec:results-text}


==> zytxnxngzdvxqhckpnjsbqvcvffzphrh/Sections/5-analysis.tex <==
\needspace{6\baselineskip}  % keep the heading with its first lines
\section{Analysis}
\label{sec:analysis}

\subsection{Rubric Efficacy}
\label{subsec:efficacy}

To intuitively demonstrate the advantages of the rubric-based method over direct judging, we fine-tune Qwen3.5-9B on two equal-sized subsets drawn from the same data pool.
\begin{figure}[!ht]
\centering
\includegraphics[width=\linewidth]{Figures/analysis/filter_ablation.pdf}
\caption{\pipename{} filtering outperforms direct-judge filtering on every benchmark.}
\label{fig:filter-ablation}
\end{figure}

One is filtered by direct scoring, where a judge assigns each
sample a single holistic score as in a typical pipeline~\citep{sun2026januscoder}, and the
other by the \pipename{} rubric. The model trained on the rubric-filtered subset scores higher on
every benchmark, by as much as 24 points on Vega-Lite (\cref{fig:filter-ablation}). The
gains are largest on the text-centric formats and small on the vision-centric benchmarks,
where Design2Code moves by a fraction of a point. Since both subsets have the same size, the gap
reflects which samples each judge keeps.

\subsection{Backbone Generalization}
\label{subsec:backbone}
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{Figures/analysis/backbone_stages.pdf}
\caption{Per-stage gains of our SFT and RL pipeline over two base models on every metric.}
\label{fig:backbone-stages}
\end{figure}
Beyond the released Qwen3.5 backbones, we apply the same data and method to
Gemma-4-31B-it~\citep{google2026gemma} and Qwen3-VL-30B-A3B-Instruct~\citep{bai2025qwen3} on
Python plotting and HTML, the two most represented domains. On both backbones all twelve metrics
end above the base model, and RL adds to SFT on every one (\cref{fig:backbone-stages}). SFT
carries most of the ChartMimic gain, whereas RL drives most of the HTML gains and recovers every
metric that dips after SFT alone. More results on Gemma are presented in Appendix~\cref{app:backbone}.

\needspace{17\baselineskip}  % keep the wrapped figure and caption on the same page
\subsection{Rubric Agreement with Humans}
\label{subsec:reliability}
\begin{wrapfigure}{r}{0.48\linewidth}
\centering
\includegraphics[width=\linewidth]{Figures/analysis/judge_agreement.pdf}
\caption{\pipename{} scoring aligns judges with humans better than direct
scoring.}
\label{fig:judge-agreement}
\end{wrapfigure}
Because multimodal code artifacts are ultimately created for humans, consistency with human judgment provides a compelling test to verify that the quality of data yielded by our rubric-based PrismaForge aligns more closely with human preferences.
At the same time, preserving the relative ordering induced by scores is particularly important for reward-based policy optimization, where inconsistent rankings can provide conflicting training signals.
To evaluate our method along both dimensions, we conducted a human study. We sampled 100 examples from our training data and asked human annotators, as well as three proprietary model judges, to evaluate them using direct scoring and the \pipename{} rubrics, respectively. We then measured the agreement between each model judge and the human ratings in terms of both absolute score levels and pairwise ordering (\cref{fig:judge-agreement}). The rubric-based judging method achieves substantially higher agreement with human judgments and greater consistency in the induced partial ordering across all three model judges. The full study protocol and detailed statistics are provided in Appendix~\cref{app:adjudication}.
We further show that the gains of our pipeline hold across judge models, with the
experiments presented in Appendix~\cref{app:backbone}.


==> zytxnxngzdvxqhckpnjsbqvcvffzphrh/Sections/6-conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this work, we push open multimodal code intelligence forward by jointly
contributing and fully releasing data, pipeline, and models. \pipename{} treats
multimodal code data under one lens with rubrics synthesized from coarse to fine
and decomposed into code-level and visual-level criteria, a signal that both
generalizes and localizes what went wrong.
We then curate and release \ourdata{}, the most broadly covering open dataset
for multimodal code intelligence, which enables principled selection and stable reinforcement learning on
visual-coding tasks. On this data we build \modelnine{}/35B, which lead the open state of the art
by a wide margin and rival proprietary systems. Extensive analyses across base models and task recipes show that the data and
the pipeline generalize beyond our release, and we share these insights and resources
to broaden access to visual-coding capabilities.


==> zytxnxngzdvxqhckpnjsbqvcvffzphrh/Tables/comparison.tex <==
% Coverage of open multimodal code-intelligence works. Sources per cell:
% writing_supp/coverage_comparison_sources.md (public papers only, read 2026-09-27).
\newcommand{\nst}{--}
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.08}
\caption{Coverage of open multimodal code-intelligence works. \cmark{} = present in the
released training corpus as its paper describes it; \xmark{} = absent from the paper;
\nst{} = not stated.}
\label{tab:comparison}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l >{\columncolor{boxblue}}c c c c c}
\toprule
& \textbf{\ourdata} & JanusCoder & VisCodex & VisCoder2 & VinciCoder \\
\midrule
\multicolumn{6}{l}{\emph{Visual code data types}} \\
Python plotting (text to plot)      & \cmark & \cmark & \nst   & \cmark & \xmark \\
Web UI (screenshot or text to page) & \cmark & \cmark & \cmark & \xmark & \cmark \\
Chart-to-code (image to code)       & \cmark & \cmark & \cmark & \xmark & \cmark \\
SVG                                 & \cmark & \cmark & \xmark & \cmark & \cmark \\
LaTeX / TikZ                        & \cmark & \xmark & \xmark & \cmark & \cmark \\
Mermaid                             & \cmark & \xmark & \xmark & \cmark & \cmark \\
Asymptote                           & \cmark & \xmark & \xmark & \cmark & \cmark \\
LilyPond                            & \cmark & \xmark & \xmark & \cmark & \xmark \\
Vega-Lite                           & \cmark & \xmark & \xmark & \cmark & \xmark \\
JavaScript                          & \cmark & \nst   & \xmark & \cmark & \xmark \\
Code-driven animation (Manim)       & \cmark & \cmark & \xmark & \xmark & \xmark \\
Interactive demos and artifacts     & \cmark & \cmark & \xmark & \xmark & \xmark \\
Chemical-structure code             & \cmark & \xmark & \xmark & \xmark & \cmark \\
Other plotting languages (R, MATLAB, C++, TS) & \xmark & \cmark & \xmark & \cmark & \xmark \\
Wolfram / Mathematica               & \xmark & \cmark & \xmark & \xmark & \xmark \\
\# visual data types covered (of 15) & \textbf{13} & 8 & 2 & 9 & 7 \\
\midrule
\multicolumn{6}{l}{\emph{Other data}} \\
General (non-visual) code           & \xmark & \cmark & \cmark & \cmark & \xmark \\
\midrule
\multicolumn{6}{l}{\emph{Artifacts and method}} \\
Released corpus                     & 2M & 800K & 598K & 679K & 1.6M \\
Open-weight models                  & 9B, 35B-A3B & 7B, 8B, 14B & \nst & 3B to 32B & 7B, 8B \\
Curation signal                     & code + vision rubrics & exec. + judge score & exec. + judge score & exec. + image checks & exec. + linters \\
Per-instruction rubric              & \cmark & \xmark & \xmark & \xmark & \xmark \\
RL stage                            & GRPO, rubric reward & \xmark & \xmark & \xmark & GRPO, visual similarity \\
Rubric as reward                    & \cmark & \xmark & \xmark & \xmark & \xmark \\
Human-agreement study of the score  & \cmark & \cmark & \xmark & \xmark & \xmark \\
\bottomrule
\end{tabular}}
\end{table}


==> zytxnxngzdvxqhckpnjsbqvcvffzphrh/Tables/main_text.tex <==
\begin{table}[t]
\centering
\footnotesize
\setlength{\tabcolsep}{4.5pt}
\caption{Text-centric results. \textbf{Best}\,/\,\underline{second} among open
models.} 
\label{tab:main-text}
\resizebox{0.92\linewidth}{!}{%
\begin{tabular}{l c ccc c c ccc}
\toprule
& \multicolumn{1}{c}{\makecell{Artifacts\\Bench}} & \multicolumn{3}{c}{PandasPlotBench}
& \multicolumn{1}{c}{\makecell{Inter-\\actSci.}} & \multicolumn{1}{c}{UniSVG}
& \multicolumn{3}{c}{VisPlotBench} \\
\cmidrule(lr){2-2}\cmidrule(lr){3-5}\cmidrule(lr){6-6}\cmidrule(lr){7-7}\cmidrule(lr){8-10}
Model
&
& \makecell{Incorr.\\Code$\downarrow$} & Visual & Task
& \makecell{PFT}
& \makecell{TSVGen}
& ExecPass & Mean & \makecell{Good\\$\geq$75} \\
\midrule
\multicolumn{10}{l}{\textit{Open models}} \\
Qwen3-VL-8B-Instruct & 34.71 & 16.00\% & 60.01 & 73.67 & 15.47\% & 68.13 & 56.52\% & 40.25 & 33.62 \\
Qwen3-VL-30B-A3B-Instruct & 41.70 & 11.43\% & 60.05 & \textbf{80.58} & 24.40\% & 69.33 & 64.38\% & 49.28 & 42.88 \\
Qwen3.5-9B & 41.24& 24.57\% & 52.98 & 65.47 & 22.40\% & 69.28 & 52.22\% & 41.18 & 36.71 \\
Qwen3.5-35B-A3B & 44.98  & 15.43\% & 60.16 & 75.17 & \underline{26.67\%} & \textbf{72.15} & 63.01\% & 51.45 & 48.51 \\
JanusCoderV-7B & 31.16 & 23.43\% & 53.05 & 65.77 & 17.73\% & 66.43 & 58.42\% & 48.10 & 32.15 \\
JanusCoderV-8B & 32.00 & 26.30\% & 56.30 & 70.91 & 17.60\% & 62.17 & 56.21\% & 47.22 & 30.87 \\
VinciCoder-7B & 11.35 & \textbf{9.14\%} & 25.37 & 51.57 & 0.40\% & 64.06 & 64.10\% & 23.95 & 10.11 \\
VinciCoder-8B & 11.97 & 12.00\% & 25.47 & 60.79 & 0.54\% & 63.45 & 63.92\% & 12.55 & 2.80 \\
VisCoder2-7B & 17.51 & 20.00\% & 59.48 & 67.59 & 1.00\% & 65.44 & \underline{66.73\%} & 49.84 & 42.50 \\
\rowcolor{boxblue} \textbf{\modelnine} & \underline{45.28} & 10.29\% & \underline{60.54} & 77.94 & 24.80\% & 68.49 & 65.30\% & \underline{53.99} & \underline{52.62} \\
\rowcolor{boxblue} \textbf{\modelthirtyfiveA} & \textbf{46.01} & \underline{9.29\%} & \textbf{62.38} & \underline{79.85} & \textbf{28.00\%} & \underline{70.72} & \textbf{71.14\%} & \textbf{62.47} & \textbf{61.49} \\
\midrule
\multicolumn{10}{l}{\textit{Proprietary}} \\
\rowcolor[gray]{0.92} \gptfouro & 33.54 & 8.00\% & 67.63 & 82.46 & 31.07\% & 72.80 & 67.99\% & 56.01 & 52.75 \\
\rowcolor[gray]{0.92} Gemini 3 Flash & 51.42 & 3.43\% & 69.95 & 91.21 & 28.13\% & 74.64 & 76.25\% & 60.92 & 58.54 \\
\rowcolor[gray]{0.92} Gemini 3.1 Pro & 53.04 & 1.71\% & 78.41 & 94.70 & 44.13\% & 74.52 & 79.57\% & 69.47 & 69.15 \\
\rowcolor[gray]{0.92} Claude Sonnet 4.6 & 64.65 & 3.43\% & 74.59 & 91.93 & 37.33\% & 74.93 & 73.00\% & 62.20 & 61.06 \\
\rowcolor[gray]{0.92} Claude Opus 4.6 & 62.47 & 1.71\% & 76.03 & 94.97 & 35.47\% & 75.47 & 73.09\% & 65.94 & 66.03 \\
\bottomrule
\end{tabular}}
\end{table}


==> zytxnxngzdvxqhckpnjsbqvcvffzphrh/Tables/main_vision.tex <==
\begin{table}[ht]
\centering
\caption{Vision-centric results. \textbf{Best}\,/\,\underline{second} among open
models.}
\label{tab:main-vision}
\setlength{\tabcolsep}{3pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{l cc ccc cc cc c c cc}
\toprule
& \multicolumn{2}{c}{ChartMimic} & \multicolumn{3}{c}{WebCode2M}
& \multicolumn{2}{c}{DesignBench} & \multicolumn{2}{c}{Design2Code}
& \multicolumn{1}{c}{\makecell{Inter-\\actSci.}} & \multicolumn{1}{c}{UniSVG}
& \multicolumn{2}{c}{ChemDraw} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-6}\cmidrule(lr){7-8}\cmidrule(lr){9-10}\cmidrule(lr){11-11}\cmidrule(lr){12-12}\cmidrule(lr){13-14}
Model
& \makecell{Low-Level} & High-Level
& \makecell{LLM\\Score} & Visual & CLIP
& Gen. & Edit.
& \makecell{LLM\\Score} & Visual
& \makecell{VQT}
& \makecell{ISVGen}
& Validity & \makecell{Tani.\\Sim.} \\
\midrule
\multicolumn{14}{l}{\textit{Open models}} \\
Qwen3-VL-8B-Instruct & 65.92 & 62.81 & 53.67 & 73.55 & 79.16 & 55.12 & 8.38 & 57.47 & 82.81 & 34.06 & 66.27 & 78.91\% & 54.79 \\
Qwen3-VL-30B-A3B-Instruct & 71.04 & 67.30 & 54.80 & 77.40 & 79.42 & 51.58 & 8.07 & 57.94 & 85.11 & 37.67 & 74.30 & 82.03\% & 54.55 \\
Qwen3.5-9B & 58.35 & 55.55 & 51.74 & 81.60 & 79.93 & 50.73 & 8.19 & 53.12 & 85.60 & 27.28 & 63.09 & 88.28\% & 66.79 \\
Qwen3.5-35B-A3B & 70.22 & 63.90 & 65.32 & 88.64 & 85.94 & 64.70 & 8.66 & 67.49 & 90.98 & 29.33 & 62.91 & 92.97\% & 79.86 \\
JanusCoderV-7B & 75.12 & 68.97 & 40.92 & 72.90 & 76.00 & 40.37 & 7.44 & 36.49 & 70.81 & 27.67 & 61.60 & 84.75\% & 72.81 \\
JanusCoderV-8B & 76.54 & 69.23 & 35.17 & 65.95 & 73.04 & 34.30 & 7.26 & 34.53 & 68.61 & 33.32 & 62.47 & 86.10\% & 76.91 \\
VinciCoder-7B & 78.30 & 66.09 & 43.11 & 72.42 & 78.59 & 43.24 & 1.40 & 42.30 & 76.64 & 0.00 & \underline{85.72} & 93.18\% & 92.15 \\
VinciCoder-8B & 77.59 & 66.44 & 46.16 & 78.26 & 80.79 & 48.09 & 1.71 & 45.72 & 81.89 & 2.33 & \textbf{87.18} & 94.21\% & 91.02 \\
\rowcolor{boxblue} \textbf{\modelnine} & \underline{81.57} & \underline{73.82} & \textbf{69.72} & \textbf{90.41} & \textbf{88.46} & \textbf{69.95} & \textbf{8.93} & \textbf{70.51} & \textbf{91.54} & \underline{51.87} & 69.64 & \underline{96.88\%} & \underline{95.94} \\
\rowcolor{boxblue} \textbf{\modelthirtyfiveA} & \textbf{83.42} & \textbf{80.69} & \underline{67.78} & \underline{89.66} & \underline{87.78} & \underline{68.98} & \underline{8.89} & \underline{67.55} & \underline{91.22} & \textbf{53.54} & 84.14 & \textbf{100.00\%} & \textbf{97.56} \\
\midrule
\multicolumn{14}{l}{\textit{Proprietary}} \\
\rowcolor[gray]{0.92} \gptfouro & 76.38 & 72.02 & 54.94 & 83.45 & 80.22 & 52.64 & 8.89 & 58.48 & 88.23 & 46.01 & 70.98 & 92.19\% & 57.80 \\
\rowcolor[gray]{0.92} Gemini 3 Flash & 85.12 & 83.04 & 69.63 & 90.41 & 87.34 & 69.28 & 9.45 & 70.12 & 92.18 & 65.25 & 82.24 & 63.28\% & 81.39 \\
\rowcolor[gray]{0.92} Gemini 3.1 Pro & 77.96 & 81.73 & 70.97 & 89.96 & 87.64 & 69.47 & 9.57 & 70.90 & 90.70 & 71.05 & 76.85 & 93.12\% & 92.45 \\
\rowcolor[gray]{0.92} Claude Sonnet 4.6 & 80.23 & 80.73 & 68.19 & 87.76 & 86.80 & 66.53 & 9.24 & 67.99 & 90.83 & 77.36 & 80.38 & 88.28\% & 85.43 \\
\rowcolor[gray]{0.92} Claude Opus 4.6 & 81.11 & 79.68 & 66.38 & 88.25 & 87.11 & 65.69 & 9.55 & 66.75 & 90.19 & 76.25 & 78.70 & 96.88\% & 77.71 \\
\bottomrule
\end{tabular}}
\vspace{-0.5em}
\end{table}


==> zytxnxngzdvxqhckpnjsbqvcvffzphrh/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> zytxnxngzdvxqhckpnjsbqvcvffzphrh/qiushi_custom.tex <==
%==============================================================================
% qiushi_custom.tex
%------------------------------------------------------------------------------
% Single source of truth for every customization layered on top of chili.cls.
% Loaded once from main.tex (after \documentclass and the general packages, and
% before cleveref so natbib is in place first).
%
%   0. Switches        -- on/off flags, edit these
%   1. Packages        -- support packages used by the features below
%   2. Colors          -- red palette + class-brand override (title/headers/links)
%   3. Abstract        -- light-red panel + optional "Abstract" heading
%   4. Headings        -- veronica-red section/subsection/.../paragraph titles
%   5. Front matter    -- optional logo area + author symbol marks
%   6. Callout box     -- tcolorbox "notebox", light-red by default
%   7. Appendix ToC    -- optional table of contents for the appendix
%   8. Macros          -- marks, notes, text shorthands (ArXiv_OSReward import)
%==============================================================================


%==============================================================================
% 0. Switches  (edit these)
%==============================================================================
\newif\ifshowabstracttitle  \showabstracttitletrue  % "Abstract" heading above the panel
\newif\ifshowlogo            \showlogofalse          % logo rides inline in \title (main.tex); header logo unused
\newif\ifnumericcite         \numericcitefalse       % true: [1] numeric | false: (Author, 2024a)
\newif\ifappendixtoc         \appendixtoctrue        % table of contents at the start of the appendix
\newif\ifanonauthors         \anonauthorsfalse       % true: byline shows only "PrismaCoder Contributors" (external review); set in main.tex


%==============================================================================
% 1. Packages
%==============================================================================
\usepackage{xspace}         % well-behaved trailing space for text macros
\usepackage{etoolbox}       % \pretocmd for the abstract heading (usually already loaded)
\usepackage{fontawesome5}   % \faEnvelope for the corresponding-author mark

% Citations. The natbib option (chosen by the switch) controls in-text style;
% the .bst (plainnat, set in main.tex) is the same for both modes.
\ifnumericcite
  \usepackage[numbers,square,sort&compress]{natbib}  % [1], [2,3]; numbered list
\else
  \usepackage[round,authoryear]{natbib}              % (Author, 2024a); round parens
  % natbib's author-year bibliography is unnumbered by default. Force numbering:
  % NAT@biblabel normally discards the (already-computed) entry number; make it
  % print, and switch to the numbered list geometry.
  \makeatletter
  \renewcommand\NAT@biblabel[1]{[#1]}
  \let\NAT@bibsetup\NAT@bibsetnum
  \makeatother
\fi

\usepackage[most]{tcolorbox}   % callout boxes (see section 6)

% Reference list: smaller font and tighter item gaps (the class parskip is generous).
\renewcommand{\bibfont}{\small}
\setlength{\bibsep}{3pt plus 1pt}

% Center table captions, including those inside minipages.
\captionsetup[table]{justification=centering}


%==============================================================================
% 2. Colors  (red theme)
%==============================================================================
% --- template look ---
\definecolor{deepred}{HTML}{A51C30}         % deep crimson: title, running headers, rules
\definecolor{AbstractRed}{HTML}{FBEDEF}     % faint rose for the abstract panel
\definecolor{boxredlight}{HTML}{FBE4E7}     % light red fill: notebox / table header / figure box
% --- imported from ArXiv_OSReward (ForestGreen/BrickRed also shadow dvipsnames) ---
\definecolor{darkblue}{rgb}{0, 0, 0.5}
\definecolor{veronica-red}{RGB}{196,30,58}  % primary red: headings, links, accents
\definecolor{ForestGreen}{RGB}{34,139,34}
\definecolor{BrickRed}{rgb}{.72,0,0}
\definecolor{LakeBlue}{RGB}{0,61,153}
\definecolor{ultramarineblue}{RGB}{18,10,143}   % blue notes: \qs/\sqs (author) + \btodo (unsure framing)
\definecolor{todored}{RGB}{222,30,30}           % red \todo: missing result/number/citation (alert red, not the heading crimson)
\definecolor{boxgreen}{rgb}{0.9,1.0,0.9}
\definecolor{boxblue}{rgb}{0.9,0.9,1.0}
\definecolor{boxred}{rgb}{1.0,0.85,0.95}
\colorlet{headingred}{veronica-red!90!black}% headings + hyperlinks; slightly deepened veronica (~#B01B34)

% --- recolor the class's brand palette to red, without editing chili.cls -------
% chili.cls references these color names at typeset time, so redefining them here
% turns the title, running headers, rules, and hyperlinks red. (The blue template
% recolors \titlefont/\headerfont inside the class; remapping the named colors keeps
% the whole red theme in this one file.)
\colorlet{BrandPrimary}{deepred}            % main title + running headers (was navy)
\colorlet{BrandRule}{deepred}               % title rule + header/footer rules (was gray)
\colorlet{BrandLink}{headingred}            % header paper URL (was link blue)
\hypersetup{linkcolor=headingred, urlcolor=headingred, citecolor=headingred}


%==============================================================================
% 3. Abstract panel
%==============================================================================
% chili.cls draws the abstract with backgroundcolor=MorandiAbstract; redirect
% that hook to the light red.
\colorlet{MorandiAbstract}{AbstractRed}

% Optional centered "Abstract" heading above the panel (switch in section 0).
% Adjust the font size here.
\newcommand{\abstractheadingfont}{\normalfont\bfseries\fontsize{14}{16}\selectfont\color{headingred}}
\makeatletter
\pretocmd{\archer@renderabstract}{%
  \ifshowabstracttitle
    {\centering\abstractheadingfont\abstractname\par}\vspace{4pt}%
  \fi
}{}{}
\makeatother


%==============================================================================
% 4. Headings -- veronica red (#C41E3A)
%==============================================================================
% Re-issue the heading formats from chili.cls, changing only the color. Sizes and
% spacing are inherited from the class; the title and headers are recolored to
% deep crimson in section 2.
\newcommand{\qsheadingfont}{\color{headingred}\bfseries\fontsize{13}{14}\selectfont}
\titleformat{\section}
  {\large\bfseries\qsheadingfont}{\thesection.}{0.5em}{#1}[]
\titleformat{name=\section,numberless}
  {\large\bfseries\qsheadingfont}{}{0em}{#1}[]
\titleformat{\subsection}
  {\color{headingred}\bfseries}{\thesubsection.}{0.5em}{#1}[]
\titleformat{\subsubsection}
  {\color{headingred}\bfseries\itshape}{\thesubsubsection.}{0.5em}{#1}[]
\titleformat{\paragraph}[runin]
  {\bfseries\color{headingred}}{\theparagraph.}{0.5em}{#1}
% Tighten \paragraph spacing: titlesec's default before-sep (3.25ex) exceeds even
% \subsection's (2.5ex); a run-in head needs little more air than a plain paragraph.
\titlespacing*{\paragraph}{0pt}{1.0ex plus 0.5ex minus .2ex}{1em}


%==============================================================================
% 5. Front matter -- optional logo area + author symbol marks
%==============================================================================
% --- Logo area: top-left of page 1, in the header above the top rule (switch in
% section 0). Holds one or more institution logos. Replace \logoblock with your
% image(s):
%   \renewcommand{\logoblock}{\includegraphics[height=9mm]{figures/logo.pdf}}
% List several \includegraphics (separated by \hspace) for multiple logos. Keep
% the height within the class headheight (40pt); raise it in chili.cls if needed.
\newcommand{\logoblock}{%
  \fcolorbox{BrandRule}{BrandLight}{\rule[-0.45em]{0pt}{1.5em}\scriptsize\itshape\,logo 1\,}\hspace{4pt}%
  \fcolorbox{BrandRule}{BrandLight}{\rule[-0.45em]{0pt}{1.5em}\scriptsize\itshape\,logo 2\,}%
}
% Put the logo into the first-page header-left without editing the class:
% snapshot the class's firststyle, then re-clone it overriding only the header.
\makeatletter
\let\ps@firststyleorig\ps@firststyle
\@namedef{f@nch@ps@firststyleorig-is-fancyhdr}{}
\makeatother
\fancypagestyle{firststyle}[firststyleorig]{\fancyhead[L]{\ifshowlogo\logoblock\fi}}

% --- Title typesetting: shrink the class's 23pt title so the (STABLE) long title
%     fits two lines instead of three. Color stays BrandPrimary (=deepred). --------
\renewcommand{\titlefont}{\color{BrandPrimary}\normalfont\bfseries\fontsize{15}{19}\selectfont}

% --- Title-block vertical air: trim the white space flanking the logo+title.
%     ABOVE the title: the 19mm logo box is the tallest item on the first line, so
%     \topskip pins its top to the text-area top; the gap up to the header rule is
%     then exactly \headsep. (A negative \vskip/\vspace* before the title cannot
%     help -- it sits at the top of the page, where TeX discards glue.) So shrink
%     \headsep to pull the rule down toward the logo. BELOW the title: the class
%     hardcodes \vskip11pt before the authors. The logo's \includegraphics box
%     reserves ~16pt of faint-glow / near-transparent margin BELOW the visible
%     prism base, so the line's reserved depth sits well under what the eye sees;
%     a NEGATIVE skip pulls the authors up into that empty band to close the gap.
%     Floor = the visible prism base (its wide bottom reaches into the author
%     column) -- keep clearance or the names collide with the logo. Patch fails
%     safe: if the class text ever stops matching, the warning fires, spacing as-is.
\geometry{headsep=14pt}   % class default 20pt; the gap between the top rule and the logo apex
% Author-year citation clusters overflow the line in a one-column layout; let TeX loosen.
\setlength{\emergencystretch}{1.5em}
\makeatletter
\renewcommand\AB@affilsepx{\protect\hspace{1em}\protect\Affilfont}
% Use the full text width for the balanced author and affiliation rows.
\patchcmd{\archer@maketitle@onecolumn}{\begin{adjustwidth}{0pt}{24pt}}{\begin{adjustwidth}{0pt}{0pt}}{}%
  {\PackageWarning{qiushi}{title width patch failed; width unchanged}}
\patchcmd{\archer@maketitle@onecolumn}{\vskip11pt}{\vskip2pt}{}%
  {\PackageWarning{qiushi}{title bottom-skip patch failed; spacing unchanged}}
\makeatother

% --- Running header (pages 2+): the class centers the full \@title, which wraps to
%     two lines. Use a single-line short title instead. (Page-1 center header is
%     empty in the class, so this affects only later pages.) -----------------------
\newcommand{\runningtitle}{PrismaCoder: Open Multimodal Code Intelligence through Decomposed Rubric Synthesis}
\fancyhead[C]{\footerfont \runningtitle}
% Clean PDF metadata (avoids a hyperref warning from the \\ in the displayed title).
\hypersetup{pdftitle={PrismaCoder: Pushing the Boundaries of Open Multimodal Code Intelligence through Decomposed Rubric Synthesis}}

% --- Author symbol marks. Use inside the \author[...] optional argument, which
%     authblk already typesets as a superscript, e.g. \author[1\equalmark]{Name},
%     \author[2\leadmark]{Name}, \author[1\corrmark]{Name}. Combine freely:
%     \author[1\leadmark\corrmark]{Name}. ---
\newcommand{\equalmark}{\ensuremath{\ast}}        % equal contribution
\newcommand{\leadmark}{\ensuremath{\dagger}}      % project lead / co-lead
\newcommand{\corrmark}{\,\faEnvelope[regular]}    % corresponding author (outline envelope; \, separates it from the affil number)

% Legend for the footer, below the contact line (see \correspondingauthor in
% main.tex). Marks are superscripts to match the author names; drop any line.
\newcommand{\authorlegend}{\upshape\footnotesize
  \textsuperscript{\ensuremath{\ast}}\,Equal contribution\quad
  \textsuperscript{\faEnvelope[regular]}\,Corresponding author}


%==============================================================================
% 6. Callout box -- light red by default, color is per-box adjustable
%==============================================================================
% Usage: \begin{notebox}[title=...] ... \end{notebox}
% Override the color for one box, e.g.:
%   \begin{notebox}[colback=boxgreen, colframe=ForestGreen!60!black, title=...]
\newtcolorbox{notebox}[1][]{%
  enhanced, breakable,
  colback=boxredlight, colframe=veronica-red, boxrule=0.5pt, arc=2pt,
  left=6pt, right=6pt, top=4pt, bottom=4pt,
  fonttitle=\bfseries, coltitle=white,
  #1
}


%==============================================================================
% 7. Appendix table of contents (optional)
%==============================================================================
% Call \appendixtoc right after \appendix in main.tex. When the switch is on it
% prints a contents list of the appendix only, via a private .apc toc file so it
% stays independent of any main \tableofcontents.
\makeatletter
\newcommand{\appendixtocname}{Appendix Contents}
\newcommand{\appendixtoc}{%
  \ifappendixtoc
    \section*{\appendixtocname}%
    \@starttoc{apc}%
    \let\qs@oldaddcontentsline\addcontentsline
    % Redirect ONLY section/subsection lines (target file "toc") into the appendix
    % TOC; drop figure/table caption lines (lof/lot) so the list isn't polluted
    % with mixed figure/table numbers.
    \renewcommand\addcontentsline[3]{%
      \def\qs@tmp{##1}\def\qs@toc{toc}%
      \ifx\qs@tmp\qs@toc \qs@oldaddcontentsline{apc}{##2}{##3}\fi}%
  \fi
}
\makeatother


%==============================================================================
% 8. Macros (ported from the ICLR 2027 submission's qiushi_custom.tex)
%==============================================================================
% Inline check / cross marks (pifont is loaded by the class).
\newcommand{\cmark}{\textcolor{ForestGreen}{\ding{51}}}
\newcommand{\xmark}{\textcolor{BrickRed}{\ding{55}}}

\newcommand{\myfont}{\fontsize{9.5}{11.5}\selectfont}

% Notes and two-tone TODOs: red = a concrete gap (missing result / number / citation);
% blue = narrative not yet settled.
\newcommand{\qs}[1]{\textcolor{ultramarineblue}{\textbf{[QS: #1]}}}
\newcommand{\sqs}[1]{\textcolor{ultramarineblue}{\textbf{[QS: #1]}}}
\newcommand{\todo}[1]{\textcolor{todored}{\textbf{[TODO: #1]}}}
\newcommand{\btodo}[1]{\textcolor{ultramarineblue}{\textbf{[TODO: #1]}}}

% Figure-3 inner-ring colors (gadgets/make_data_pie.py), used as swatches in the
% statistics table so the table doubles as the pie's legend.
\definecolor{pievision}{HTML}{DA8A9C}
\definecolor{pietext}{HTML}{8FA8C8}
\newcommand{\swatch}[1]{\textcolor{#1}{\rule{0.85em}{0.85em}}\,}

% Canonical names. Never hyphenate the product names.
\hyphenation{PrismaCoder PrismaForge}
\newcommand{\methodname}{\textsc{PrismaCoder}\xspace}
\newcommand{\pipename}{\textsc{PrismaForge}\xspace}
\newcommand{\modelnine}{\textsc{PrismaCoder}-9B\xspace}
\newcommand{\modelthirtyfive}{\textsc{PrismaCoder}-35B\xspace}
\newcommand{\modelthirtyfiveA}{\textsc{PrismaCoder}-35B-A3B\xspace}
\newcommand{\ourdata}{\textsc{PrismaCoder}-2M\xspace}
\newcommand{\vut}{Visual Unit Test\xspace}
\newcommand{\geminipro}{\texttt{Gemini-3-Pro}\xspace}
\newcommand{\claudeopus}{\texttt{Claude-Opus-4.6}\xspace}
\newcommand{\gptfouro}{\texttt{GPT-4o}\xspace}

% Inline model logos (Figures/icons/) for table rows and captions.
\newcommand{\gemmaicon}{\raisebox{-0.15em}{\includegraphics[height=0.9em]{Figures/icons/Gemma_icon.png}}\,}
\newcommand{\qwenicon}{\raisebox{-0.15em}{\includegraphics[height=0.9em]{Figures/icons/Qwen.png}}\,}

% Case-study panels (appendix): one image + label, for strips of any width.
\newcommand{\casepanel}[4][\footnotesize]{\begin{minipage}[t]{#4}\centering
\includegraphics[width=\linewidth]{Figures/case_studies/#2}\\[2pt]
{#1 #3}\end{minipage}}
\newcommand{\casepanelh}[5][\footnotesize]{\begin{minipage}[t]{#4}\centering
\includegraphics[width=\linewidth,height=#5,keepaspectratio]{Figures/case_studies/#2}\\[2pt]
{#1 #3}\end{minipage}}

% Case-study triptych: gold | baseline | ours, equal-width columns.
\newcommand{\casetriptych}[5]{%
\begin{figure}[htbp]
\centering
\begin{minipage}[t]{0.32\linewidth}\centering
\includegraphics[width=\linewidth]{Figures/case_studies/#1_gold.png}\\[2pt]
{\footnotesize Gold}
\end{minipage}\hfill
\begin{minipage}[t]{0.32\linewidth}\centering
\includegraphics[width=\linewidth]{Figures/case_studies/#1_baseline.png}\\[2pt]
{\footnotesize #2}
\end{minipage}\hfill
\begin{minipage}[t]{0.32\linewidth}\centering
\includegraphics[width=\linewidth]{Figures/case_studies/#1_ours.png}\\[2pt]
{\footnotesize #3}
\end{minipage}
\caption{#4}
\label{#5}
\end{figure}}

% Dash-row helpers for the appendix result tables: a run of "--" cells.
\newcommand{\dthree}{& -- & -- & --}
\newcommand{\dfour}{& -- & -- & -- & --}
\newcommand{\dfive}{& -- & -- & -- & -- & --}
\newcommand{\dsix}{& -- & -- & -- & -- & -- & --}
\newcommand{\dseven}{& -- & -- & -- & -- & -- & -- & --}
\newcommand{\deight}{& -- & -- & -- & -- & -- & -- & -- & --}

% Figure palette (Fig. 2 lanes; App. C prompt boxes): slate blue / clay / plum / mint.
\definecolor{figCurLine}{HTML}{6D8ABE}
\definecolor{figCurFill}{HTML}{EEF3FA}
\definecolor{figRlLine}{HTML}{D78C6E}
\definecolor{figRlFill}{HTML}{FBF2EC}
\definecolor{figRubLine}{HTML}{8E6AA8}
\definecolor{figRubFill}{HTML}{F5F0F7}
\definecolor{figNodeLine}{HTML}{B5B9C4}
\definecolor{figDataLine}{HTML}{4E9C87}
\definecolor{figDataFill}{HTML}{DDF3EC}
\definecolor{figCodeLine}{HTML}{9DB4DA}
\definecolor{figCodeFill}{HTML}{DCE8F8}
\definecolor{figVisLine}{HTML}{8FC9BB}
\definecolor{figVisFill}{HTML}{D6EFE8}

